Counterexamples to the $p(t)$-adic Littlewood Conjecture Over Small Finite Fields

In 2004, de Mathan and Teuli\'e stated the $p$-adic Littlewood Conjecture ($p$-$LC$) in analogy with the classical Littlewood Conjecture. Given a field $\mathbb{K}$ and an irreducible polynomial $p(t)$ with coefficients in $\mathbb{K}$, $p$-$LC$ admits a natural analogue over function fields, abbreviated to $p(t)$-$LC$ (and to $t$-$LC$ when $p(t)=t$). In this paper, an explicit counterexample to $p(t)$-$LC$ is found over fields of characteristic 5. Furthermore, it is conjectured that this Laurent series disproves $p(t)$-$LC$ over all fields of characteristic $p\equiv 1 \mod 4$. This fills a gap left by a breakthrough paper from Adiceam, Nesharim and Lunnon (2022) in which they conjecture $t$-$LC$ does not hold over all complementary fields of characteristic $p\equiv 3\mod 4$ and proving this in the case $p=3$. Supported by computational evidence, this provides a complete picture on how $p(t)$-$LC$ is expected to behave over all fields with characteristic not equal to 2. Furthermore, the counterexample to $t$-$LC$ over fields of characteristic 3 found by Adiceam, Nesharim and Lunnon is proven to also hold over fields of characteristic 7 and 11, which provides further evidence to the aforementioned conjecture. Following previous work in this area, these results are achieved by building upon combinatorial arguments and are computer assisted. A new feature of the present work is the development of an efficient algorithm (implemented in Python) that combines the theory of automatic sequences with Diophantine approximation over function fields. This algorithm is expected to be useful for further research around Littlewood-type conjectures over function fields.

==> junk.tex <==

\begin{example}
In this case,   \begin{align*}
    &\tau'(0)=\begin{matrix}
        &0&0&\\0&0&0&0\\&0&0&
    \end{matrix}& &\tau'(1)=\begin{matrix}
        &1&1&\\1&1&1&1\\&1&1&
    \end{matrix}& \tau'\left(\phi^1(0)\right)=\tau'\left(\begin{matrix}
            \color{red}0&\color{blue}1\\\color{green}1&\color{black}0
        \end{matrix}\right)= \begin{matrix}
            &&&\color{blue}1&\color{blue}1&&&&\\
            &&\color{blue}1&\color{blue}1&\color{blue}1&\color{blue}1&&&\\
            &\color{red}0 &\color{red}0 &\color{blue}1&\color{blue}1&\color{black}0&\color{black}0\\
            \color{red}0&\color{red}0&\color{red}0&\color{red}0&\color{black}0&\color{black}0&\color{black}0&\color{black}0\\
            &\color{red}0 &\color{red}0 &\color{green}1&\color{green}1&\color{black}0&\color{black}0\\
            &&\color{green}1&\color{green}1&\color{green}1&\color{green}1&&\\
            &&&\color{green}1&\color{green}1&&&&
        \end{matrix}
\end{align*}
\noindent In this example, a 45 degrees anticlockwise `rotation' is carried out before applying $\tau'$. This is a matter of presentation and noes not change any fundamental properties of the sequence. In fact, such rotations greatly aid in the understanding of how number walls can be thought of as automatic sequences.
\end{example}

The following subsection details why the notion of automaticity described by Figure \ref{auto_nw} is likely to be the correct one.


\subsection{Discussion of Conjecture \ref{autonw}}
\noindent Let $\Sigma$ be a finite alphabet, $\phi:\Sigma^*\to\Sigma^*$ be a uniform $k$-morphism for some $k\in\N$ and let $\sigma_0$ be $\phi$-prolongable. Additionally, let $\tau:\Sigma\to\F_q^{n}$ be a coding for some even $n\in\N$. As per Figure \ref{tile_fig}, the number wall of $\tau(\phi^\omega(\sigma_0))$ is split into tiles. Then, one can define a coding $$\mathcal{C}:\left\{\text{subwords of }\phi^\omega(\sigma_0)\right\}\to \left\{\text{tiles of }W_q(\tau(\phi^\omega(\sigma_0)))\right\}$$ as follows. \\

\noindent First, define $C(\epsilon)$ to be the tile comprised entirely of zeroes. Next, let $T$ be a tile that comprises part of the zeroth row of the number wall of $W_q(\tau(\phi^\omega(\sigma_0)))$. Then, if $\sigma\in\Sigma$ is such that $T=W_q(\tau(\sigma))$, define $\mathcal{C}(\sigma)=T$. Furthermore, if $w$ is a subword of $\phi^\omega(\sigma_0)$ with length greater than 1, then let $T$ be the unique tile that appears in $W_q(\tau(w))$ but not $W_q(\tau(w'))$ for any $w'$ a subword of $w$. Define $\mathcal{C}(w)=T$. If $w$ has length $r\in\N$, then $T$ is a \textit{tile of order} $r$. This coding is illustrated below. \begin{figure}[H]
\begin{center}
    \includegraphics[width=0.40\linewidth]{Tile_labeling.PNG}
    \caption{$\mathcal{C}(\sigma_i\sigma_j\sigma_k)$ is the lowest outlined tile (blue, labelled with $\sigma_i\sigma_j\sigma_k$), as it appears in $W_q(\tau(\sigma_i\sigma_j\sigma_k))$ but not in $W_q(\tau(\sigma_i\sigma_j))$, $W_q(\tau(\sigma_j\sigma_k))$, $W_q(\tau(\sigma_i))$, $W_q(\tau(\sigma_j))$ or $W_q(\tau(\sigma_k))$. This tile is of order 3.\label{ABA}}
      \vspace{-1.5em}
\end{center}
\end{figure}
\noindent The coding $\mathcal{C}$ is not injective, since the set of tiles comprising $W_q(\tau(\phi^\omega(\sigma_0)))$ is finite and the set of subwords of $\phi^\omega(\sigma_0)$ is infinite.\\

\noindent Applying $\phi$ to the tiles of order zero (in the natural way via the above association) induces a two-dimensional $k$-morphism $\Phi:\Sigma^*\to (\Sigma^*)^{k^2}$ on subwords in $\Sigma^*$. To state $\Phi$, let $a,b\le k-1$ be integers and let $w$ be a finite word in $\Sigma^*$. Then, define $\phi_{a,b}(w)$ as the subword $\phi(w)$ with the first $a$ letters and the last $b$ letters removed. Hence, applying $\phi_{a,b}$ to any subword $w$ of length $l$ creates a subword of length $kl-a-b$. Therefore, if $kl-a-b>l$, $\phi_{a,b}$ increases the length of the subword. Since $a+b\le 2(k-1)$, this is always true when $l>2(k-1)$. In particular, applying $\phi_{a,b}$ such that $a+b=k-1$ to an entry of $\Sigma$ will return another entry of $\Sigma$, and $\phi_{k-1,k-1}$ applied to a subword of length 2 will return a subword of length 2. Applying $\phi_{a,b}$ such that $a+b>k$ to a subword of length 1 returns the empty word $\epsilon$ by definition. The two-dimensional $k$-morphism $\Phi$ is then defined as below.

\begin{figure}[H]
\begin{center}
    \includegraphics[scale=0.85]{k_morph.png}
    \caption{\label{k-morph}The two-dimensional $k$-morphism induced by $\phi$. Recall that the morphism $\Phi$ only involves the \textit{subwords}, not the tiles. The tiles are illustrated here depict $\Phi(w)$ under the coding $\mathcal{C}$. }
      \vspace{-1.5em}
      \label{two_dim_morph}
\end{center}
\end{figure}
\noindent  The following lemma verifies that $\Phi$ generates the number wall of $\tau(\phi^\omega(\sigma_0))$. \begin{lemma}\label{equal}
    Let $k$ be a natural number, $\phi:\Sigma^*\to\Sigma^*$ be a uniform $k$-morphism on a finite alphabet $\Sigma$, $\sigma_0\in\Sigma$ be $\phi$-prolongable and let $\tau:\Sigma\to\F_q^{d}$ be a coding for some even natural number $d$. Then, with $\mathcal{C}$ and $\Phi$ as defined above, \begin{equation*}
        \mathcal{C}(\Phi^\omega(\sigma_0))=W_q(\tau(\phi^\omega(\sigma_0))).
    \end{equation*}
\end{lemma}
\noindent As the content of this section is speculative, only an abridged version of the proof is provided here.
\begin{proof}[Abridged Proof]
    First, one must verify that $\Phi^\omega(\sigma_0)$ is well defined. Indeed, $\sigma_0$ is $\Phi$-prolongable because $\sigma_0$ is $\phi$-prolongable and hence $\phi_{0,k-1}(\sigma_0)=\sigma_0$.\\

    \noindent The goal is to show that $\mathcal{C}(\Phi^n(\omega))=W_q(\tau(\phi^n(\sigma_0))$ for all $n\in\N$. The proof proceeds by induction. For the base case, $\mathcal{C}(\sigma_0)=W_q(\tau(\sigma_0))$ by definition. Next, assume $w$ is a subword of length $r\in\N$ inside $\phi^n(\sigma_0)$. For $1\le i \le r$, let $w_i$ denotes the $i^\nth$ letter of $w$. The tile associated to $w$ is depicted below. \begin{figure}[H]
        \centering
        \includegraphics[width=0.3\linewidth]{m1.PNG}
        \caption{The red, blue and green tiles are given by $\mathcal{C}(w_1)$, $\mathcal{C}(w_r)$ and $\mathcal{C}(w)$ respectively. The rest of the number wall is omitted for the sake of clarity. The horizontal black line is in place of the tiles associated to $w_i$ for $2\le i \le r-1$, and similarly the diagonal lines are in place of other tiles.}
    \end{figure} \noindent Applying $\phi$ to $w$ attains a word of length $k\cdot r$, denoted $\phi(w)$ and equal to $\phi(w_1)\phi(w_2)\cdots\phi(w_r)$. The number wall $W_q(\tau(\phi(w)))$ admits a natural partition into $r^2$ pieces, each of which is defined to be the image of some subword $w'$ of $w$ under $\Phi$. Each of these parts then splits into $k^2$ tiles, as depicted below.  \begin{figure}[H]
        \centering
        \includegraphics[width=1\linewidth]{m2.PNG}
        \caption{The number wall of $\phi(w)$ is split into $r^2$ pieces, three of which are coloured in the above diagram. In particular, the image of $w_1$, $w_2$ and $w$ under $\Phi$ is drawn in red, blue and green respectively. Each is a $k\times k$ rotated square of tiles. The parts corresponding to $\Phi(w_1)$ and $\Phi(w_2)$ have had all tiles relating to rows of the number wall with negative index removed. Then, $\Phi(w)$ is split into $k^2$ tiles.}
        \label{m2}
    \end{figure}
\noindent The goal is now to show that the portion of the number wall in green in Figure \ref{m2} agrees with the image of $w$ under $\Phi$ as defined in Figure \ref{two_dim_morph}. Indeed, for a given tile $T$ inside $\Phi(w)$, there exists a minimal-length subword $w'$ of $\phi(w)$ such that $T$ appears in $W_q(\tau(w'))$. Furthermore, as $T$ is in $\Phi(w)$, $w'$ is equal to $\phi(w)$ with $a$ entries removed from the start and $b$ entries removed from the end, for some $0\le a,b<k$. Note that if $a\ge k$, this would imply that a tile within $\Phi(w)$ does not depend on either $w_1$ which implies that $w_1$ is not the first letter of $w$, which is a contradiction. Similarly for $b\ge k$ and $w_r$. Considering all possible $0\le a,b \le k-1$ completes the proof.
\end{proof}

\noindent As there are infinitely many finite subwords of $S$, and only finitely many possible tiles (as the entries of the number wall are in $\F_q$), it is not obvious that $\mathcal{C}(\Phi^\omega(\sigma_0))$ should be a two-dimensional $k$-automatic sequence. Indeed, given a tile $T$, one can find a set of finite words $\Sigma_T\subset\Sigma^*$ such that every $w\in\Sigma_T$ satisfies $\mathcal{C}(w)=T$. Furthermore, as the set of all possible tiles $T$ is finite, one can partition $\Sigma$ into finitely many disjoint subsets: \[\Sigma=\bigsqcup_{T}\Sigma_T,\] where the above union is taken over all possible tiles. However, there is no immediate reason why, for any given natural numbers $a,b<k-1$ and subwords $w_1,w_2\in \Sigma_T$, there should exist some tile $T'$ such that both $\phi_{a,b}(w_1),\phi_{a,b}(w_2)$ should belong to $\Sigma_{T'}$. Satisfying this would immediately imply that $C(\Phi^\omega(\sigma_0))$ is a two dimensional $k$-automatic sequence, as $\Phi$ would be a uniform $k$-morphism on the finite alphabet formed by taking natural equivalence classes on $\Sigma$. The main obstacle in the way of attaining Conjecture \ref{autonw} is in proving this statement. 

\noindent One now defines a coding $$\mathcal{C}:\left\{\text{subwords of }\phi^\omega(\sigma_0)\right\}\to \left\{\text{tiles of }W_q(\tau(\phi^\omega(\sigma_0)))\right\}.$$ Let $T$ be a tile that comprises part of the zeroth row of the number wall of $W_q(\tau(\phi^\omega(\sigma_0)))$. Then, if $\sigma\in\Sigma$ is such that $T=W_q(\tau(\sigma))$, define $\mathcal{C}(\sigma)=T$. Furthermore, if $w$ is a subword of $\phi^\omega(\sigma_0)$ with length greater than 1, then let $T$ be the unique tile that appears in $W_q(\tau(w))$ but not $W_q(\tau(w'))$ for any $w'$ a subword of $w$ and define $\mathcal{C}(w)=T$. If $w$ has length $r\in\N$, then $T$ is a \textit{tile of order} $r$. This coding is illustrated below. \begin{figure}[H]
\begin{center}
    \includegraphics[scale=0.5]{Tile_labeling.PNG}
    \caption{$\mathcal{C}(\sigma_i\sigma_j\sigma_k)$ is the lowest outlined tile (blue, labelled with $\sigma_i\sigma_j\sigma_k$), as it appears in $W_q(\tau(\sigma_i\sigma_j\sigma_k))$ but not in $W_q(\tau(\sigma_i\sigma_j))$, $W_q(\tau(\sigma_j\sigma_k))$, $W_q(\tau(\sigma_i))$, $W_q(\tau(\sigma_j))$ or $W_q(\tau(\sigma_k))$. This tile is of order 3.\label{ABA}}
      \vspace{-1.5em}
\end{center}
\end{figure}
\noindent It is necessary that there exist at least two different subwords $w_1$ and $w_2$ such that $\mathcal{C}(w_1)=\mathcal{C}(w_2)$, since the set of tiles comprising $W_q(\tau(\phi^\omega(\sigma_0)))$ is finite and the set of subwords of $\phi^\omega(\sigma_0)$ is infinite.\\

\noindent Applying $\phi$ to the tiles of order zero (in the natural way via the above association) induces a two-dimensional $k$-morphism $\Phi:\Sigma^*\to (\Sigma^*)^{k^2}$ on subwords in $\Sigma^*$. To state $\Phi$, let $a,b\le k-1$ be integers and let $w$ be a finite word in $\Sigma^*$. Then, define $\phi_{a,b}(w)$ as the subword $\phi(w)$ with the first $a$ letters and the last $b$ letters removed. Hence, applying $\phi_{a,b}$ to any subword $w$ of length $l$ creates a subword of length $kl-a-b$. Therefore, if $kl-a-b>l$, $\phi_{a,b}$ increases the length of the subword. Since $a+b\le 2(k-1)$, this is always true when $l>2(k-1)$. In particular, applying $\phi_{a,b}$ such that $a+b=k-1$ to an entry of $\Sigma$ will return another entry of $\Sigma$, and $\phi_{k-1,k-1}$ applied to a subword of length 2 will return a subword of length 2. Applying $\phi_{a,b}$ such that $a+b>k$ to a subword of length 1 returns the empty word $\epsilon$ by definition. The two-dimensional $k$-morphism $\Phi$ is then defined as below.

\begin{figure}[H]
\begin{center}
    \includegraphics[scale=0.85]{k_morph.png}
    \caption{\label{k-morph}The two-dimensional $k$-morphism induced by $\phi$. Recall that the morphism $\Phi$ only involves the \textit{subwords}, not the tiles. The tiles are illustrated here depict $\Phi(w)$ under the coding $\mathcal{C}$. }
      \vspace{-1.5em}
      \label{two_dim_morph}
\end{center}
\end{figure}
\noindent  The following lemma verifies that $\Phi$ generates the number wall of $\tau(\phi^\omega(\sigma_0))$. \begin{lemma}\label{equal}
    Let $k$ be a natural number, $\phi:\Sigma^*\to\Sigma^*$ be a uniform $k$-morphism on a finite alphabet $\Sigma$, $\sigma_0\in\Sigma$ be $\phi$-prolongable and let $\tau:\Sigma\to\F_q^{d}$ be a coding for some even natural number $d$. Then, with $\mathcal{C}$ and $\Phi$ as defined above, \begin{equation*}
        \mathcal{C}(\Phi^\omega(\sigma_0))=W_q(\tau(\phi^\omega(\sigma_0))).
    \end{equation*}
\end{lemma}
\noindent Only an abridged version of the proof of Lemma \ref{equal} is provided, since the algorithms used to prove theorems \ref{F5} and \ref{F7} verify it in the cases required.
\begin{proof}
    First, one must verify that $\Phi^\omega(\sigma_0)$ is well defined. Indeed, $\sigma_0$ is $\Phi$-prolongable because $\sigma_0$ is $\phi$-prolongable and hence $\phi_{0,k-1}(\sigma_0)=\sigma_0$.\\

    \noindent The goal is to show that $\mathcal{C}(\Phi^n(\omega))=W_q(\tau(\phi^n(\sigma_0))$ for all $n\in\N$. The proof proceeds by induction. For the base case, $\mathcal{C}(\sigma_0)=W_q(\tau(\sigma_0))$ by definition. Next, assume $w$ is a subword of length $r\in\N$ inside $\phi^n(\sigma_0)$. For $1\le i \le r$, let $w_i$ denotes the $i^\nth$ letter of $w$. The tile associated to $w$ is depicted below. \begin{figure}[H]
        \centering
        \includegraphics[width=0.3\linewidth]{m1.PNG}
        \caption{The red, blue and green tiles are given by $\mathcal{C}(w_1)$, $\mathcal{C}(w_r)$ and $\mathcal{C}(w)$ respectively. The rest of the number wall is omitted for the sake of clarity. The horizontal black line is in place of the tiles associated to $w_i$ for $2\le i \le r-1$, and similarly the diagonal lines are in place of other tiles.}
    \end{figure} \noindent Applying $\phi$ to $w$ attains a word of length $k\cdot r$, denoted $\phi(w)$ and equal to $\phi(w_1)\phi(w_2)\cdots\phi(w_r)$. The number wall $W_q(\tau(\phi(w)))$ admits a natural partition into $r^2$ pieces, each of which is defined to be the image of some subword $w'$ of $w$ under $\Phi$. Each of these parts then splits into $k^2$ tiles, as depicted below.  \begin{figure}[H]
        \centering
        \includegraphics[width=1\linewidth]{m2.PNG}
        \caption{The image of $w_1$, $w_2$ and $w$ under $\Phi$ is drawn in red, blue and green respectively. Each is a $k\times k$ rotated square of tiles. $\Phi(w_1)$ and $\Phi(w)_2$ have had all tiles relating to rows of the number wall with negative index removed. Then, $\Phi(w)$ is split into $k^2$ tiles and the subword which an arbitrary tile corresponds to is calculated.}
    \end{figure}
\noindent The goal is now to show that this definition of $\Phi$ agrees with Figure \ref{two_dim_morph}. Indeed, for a given tile $T$ inside $\Phi(w)$, there exists a minimal-length subword $w'$ of $\phi(w)$ such that $T$ appears in $W_q(\tau(w'))$. Furthermore, as $T$ is in $\Phi(w)$, $w'$ is equal to $\phi(w)$ with $a$ entries removed from the start and $b$ entries removed from the end, for some $0\le a,b<k$. Note that if $a\ge k$, this would imply that a tile within $\Phi(w)$ does not depend on either $w_1$ which implies that $w_1$ is not the first letter of $w$, which is a contradiction. Similarly for $b\ge k$ and $w_r$.  
\noindent 
\end{proof}

\noindent As there are infinitely many finite subwords of $S$, and only finitely many possible tiles (as the entries of the number wall are in $\F_q$), it is not obvious that $\mathcal{C}(\Phi^\omega(\sigma_0))$ should be a two-dimensional $k$-automatic sequence. Indeed, given a tile $T$, one can find a set of finite words $\Sigma_T\subset\Sigma^*$ such that every $w\in\Sigma_T$ satisfies $\mathcal{C}(w)=T$. Furthermore, as the set of all possible tiles $T$ is finite, one can partition $\Sigma$ into finitely many disjoint subsets: \[\Sigma=\bigsqcup_{T}\Sigma_T,\] where the above union is taken over all possible tiles. However, there is no reason \textit{a priori} why, for any given natural numbers $a,b<k-1$ and subwords $w_1,w_2\in \Sigma_T$, there should exist some tile $T'$ such that both $\phi_{a,b}(w_1),\phi_{a,b}(w_2)\in\Sigma_{T'}$. Satisfying this condition would immediately imply that $C(\Phi^\omega(\sigma_0))$ is a two dimensional $k$-automatic sequence, as $\Phi$ would be a uniform $k$-morphism on the finite alphabet formed by taking natural equivalence classes on $\Sigma$. The heart of the proof of Theorems \ref{F5} and \ref{F7} is in proving that, for the First and Second Level Paperfolding Sequences over the stated fields $\F_q$, $\Phi$ is indeed a two dimensional $k$-automatic sequence. 













\begin{figure}[H]
        \centering
        \includegraphics[width=1\linewidth]{morph-proof.PNG}
        \caption{\textbf{Left:} The portion of $W_q(\tau(\phi^\omega(\sigma_0)))$ generated by the subword $w=\sigma_i\sigma_j\sigma_k\sigma_l$. \textbf{Right:} The portion of $W_q(\tau'(\phi^\omega(\sigma_0)))$ generated by the same subword. Each tile of $\mathcal{C'}(w)$ is split into $k^2$ (here, $k=2$) tiles, all of which are drawn in similar colours. For example, $\sigma_i$ is sent to the four subwords whose image under $\mathcal{C}$ comprise $\mathcal{C}'(\sigma_i)$. }
    \end{figure}

    Next, consider the number wall of $\phi^\omega(\sigma_0)$ when $\tau$ is replaced with its $k$-compression, $\tau'$. As $\phi^\omega(\sigma_0)$ is fixed under $\phi$, one has that $W_q(\tau(\phi^\omega(\sigma_0)))=W_q(\tau'(\phi^\omega(\sigma_0)))$. Therefore, one obtains two different codings, $\mathcal{C}$ and $\mathcal{C}'$. However, the tiles that comprise $W_q(\tau'(\phi^\omega(\sigma_0)))$ are $k$ times the size of the tiles that comprise $W_q(\tau(\phi^\omega(\sigma_0)))$. Therefore, each can be split into $k^2$ tiles from $W_q(\tau(\phi^\omega(\sigma_0)))$, which defines a two-dimensional $k$-morphism as follows.

To begin the primary tile computing function, enough pre-computed tiles from the start of the number wall must be provided as input to `kickstart' the process. Specifically, the \texttt{input\textunderscore generator} function generates all of the unique tiles along the zeroth row of the number wall, using the sequence itself to form this input. In the case of the Paperfolding Sequence, this process also generates four tiles from the row below. By computing every unique tile on the zeroth row of the number wall before the main tiling function, the complexity of said function can be reduced significantly. This is because every tile below the zeroth row can be computed using the exact same algorithm (described in \hyperref[12]{Algorithm 1.2: Completing ${\Phi_{pf,p}}$}).\\

Each of these Tiles are then added to \texttt{tiles} and \texttt{tiles\textunderscore by\textunderscore index}. Finally, the \texttt{input\textunderscore generator} function calculates the image of each Tile on the zeroth row by applying {\fontfamily{cmtt}\selectfont\textbf{Step 1.1.3}}. The \texttt{value} for each image Tile is populated using a scaled-down version of the scaffolding technique demonstrated in Figure \ref{1.2}, where the scaffolding surrounding each image Tile is populated by retrieving Tiles from the \texttt{tiles\textunderscore by\textunderscore index} list through using $\phi$ to identify Tile indexes in the list. The top Tile of the scaffolding is always the \texttt{First Tile} for image Tiles on the zeroth row.

\noindent This result was complemented in 2023 when the second named author \cite{My_paper} proved the following theorem:\begin{theorem}\label{my_result}
    Let $\Theta(t)=\sum_{i=1}^\infty a_it^{-i}\in\F_q((t^{-1}))$ be a counterexample to the $t$-$LC$ and let $p(t)\in\F_q[t]$ be an irreducible polynomial. Then $\Theta(p(t))=\sum_{i=1}^\infty a_i p(t)^{-i}\in\F_q((t^{-1}))$ is a counterexample to $p(t)$-LC.
\end{theorem} \noindent Combining Theorems \ref{F3} and \ref{my_result} gives the corollary that $p(t)$-$LC$ is false over fields of characteristic 3 for any choice of irreducible polynomial $p(t)$. \\

\noindent The following definition is required to state the main results of this paper. \begin{definition}Let $n$ be a natural number and $k_n$ be as it was in (\ref{pfseq}). The \textit{Modified Paperfolding Sequence} is defined as \begin{equation}\label{apf1}
    g_n=\begin{cases}0 &\text{ if }k_n\equiv 1 \mod 8\\
    1 &\text{ if }k_n\equiv 3 \mod 8\\
    2 &\text{ if }k_n\equiv 5 \mod 8\\
    3 &\text{ if }k_n\equiv 7 \mod 8,\end{cases}
\end{equation} \end{definition}

\noindent Extending Theorem \ref{F3}, it is conjectured in \cite{Faustin} that the Paperfolding Sequence provides counterexample to $t$-$LC$ over fields of characteristic $p\equiv 3\mod 4$. In this paper, this conjecture is confirmed for fields of characteristic 7 and 11. However, the authors of \cite{Faustin} were unable to find a sequence that provided a counterexample to $t$-$LC$ in fields of characteristic $p\equiv 1\mod 4$. This paper fills this gap by providing a sequence that is a counterexample to $p(t)$-$LC$ over $\F_5$ for any choice of irreducible polynomial $p(t)$, thus giving the main result of this paper:
\begin{theorem}\label{main}
    The $p(t)$-$LC$ is false over fields of characteristic 0,3,5,7 and 11.
\end{theorem}
\noindent Furthermore, strong empirical evidence is provided the same sequence disproves $p(t)$-$LC$ when the characteristic of the ground field is congruent to 1 modulo 4. This conjecture provides the complementary case to the conjecture of Adiceam, Nesharim and Lunnon. When the two conjectures are taken in combination, they provide an almost complete picture of how $p(t)$-$LC$ fails in all finite fields. 
\begin{conjecture}\label{main_conj}
Let $p$ be a prime and let $\mathbb{K}$ be a field of characteristic $p$.
    \begin{enumerate}
        \item If $p=2$ and $\mathbb{K}=\mathbb{F}_2$, then $p(t)$-$LC$ is true for every irreducible $p(t)\in\mathbb{F}_2[t]$.
        \item If $p\equiv 1 \mod 4$, then the Paperfolding Sequence provides a counterexample to $p(t)$-$LC$ over $\mathbb{K}$.
        \item If $p\equiv 3 \mod 4$, then the Modified Paperfolding Sequence provides a counterexample to $p(t)$-$LC$ over $\mathbb{K}$.
    \end{enumerate}
\end{conjecture}
\noindent Evidence for statement 1 is provided in Section \ref{sect:end}, along with a discussion of the missing case where $\mathbb{K}$ is a field of even characteristic with cardinality greater than 2.\\

\noindent The proof of Theorem \ref{main} is achieved by rephrasing $t$-$LC$\footnote{Recall that Theorem \ref{my_result} implies disproving $t$-$LC$ is sufficient to disprove $p(t)$-$LC$ for any irreducible polynomial $p(t)$} in terms of the so-called \textit{number wall} of a sequence, which is defined in Section \ref{section2}. For the purposes of this introduction, the number wall of a one dimensional sequence $S$ is a two dimensional sequence derived from $S$. The core idea used to prove Theorem \ref{main} is similar to that used by Adiceam, Nesharim and Lunnon in \cite{Faustin}. That is, the number wall is shown to be the limiting sequence of a 2-morphism applied to a finite set of tiles. Both the 2-morphism and the tiles are provided explicitly. The implementation of their algorithm can be found at \cite{Fred_Code} and \cite{erez_code}. Theoretically, the algorithm used in \cite{Faustin} could be used to obtain Theorem \ref{main}. However, the time it would take to do so is outside the scope of a human lifetime. In this paper, two key improvements are made that allow for the proof of Theorem \ref{main} with only a month of runtime. Firstly, the shape of the tiles used has been changed from \cite{Faustin}, decreasing the number of tiles needed to tile the number wall of the Paperfolding sequence over $\F_3$ by an order of magnitude. Furthermore, a new algorithm has been created that finds these tiles in a far more efficient way. 

 Its statement relies on the following definition:

\begin{definition} Let $n$ be a natural number and let $k_n:=\max_{k\in\N}\{k: k|n \text{ and }2\not|k\}$ . Define the \textit{Paperfolding Sequence} as\begin{equation}\label{pfseq}
    f_n=
    \begin{cases}
        0 &\text{ if }k_n\equiv 1 \mod 4\\
        1 &\text{ if }k_n\equiv 3 \mod 4.
    \end{cases}
\end{equation}\end{definition} 
\begin{theorem}[Adiceam, Nesharim and Lunnon, 2021]\label{F3}
    The Laurent series whose coefficients are given by the Paperfolding Sequence is a counterexample to $t$-$LC$ over finite fields of characteristic 3. 
\end{theorem}

